A Quantitative Approach for Adopting Disaggregated Memory in HPC Systems

Memory disaggregation has recently been adopted in data centers to improve resource utilization, motivated by cost and sustainability. Recent studies on large-scale HPC facilities have also highlighted memory underutilization. A promising and non-disruptive option for memory disaggregation is rack-scale memory pooling, where shared memory pools supplement node-local memory. This work outlines the prospects and requirements for adoption and clarifies several misconceptions. We propose a quantitative method for dissecting application requirements on the memory system from the top down in three levels, moving from general, to multi-tier memory systems, and then to memory pooling. We provide a multi-level profiling tool and LBench to facilitate the quantitative approach. We evaluate a set of representative HPC workloads on an emulated platform. Our results show that prefetching activities can significantly influence memory traffic profiles. Interference in memory pooling has varied impacts on applications, depending on their access ratios to memory tiers and arithmetic intensities. Finally, in two case studies, we show the benefits of our findings at the application and system levels, achieving 50% reduction in remote access and 13% speedup in BFS, and reducing performance variation of co-located workloads in interference-aware job scheduling.

==> backup/background.tex <==
\section{Background}
\todo{definition of disaggregated memory, refer to the survey~\cite{ewais_disaggregated_2023}}The key idea of a memory server is to pool memory resources to be shared among multiple nodes, to enable peak-of-sums provisioning rather than sum-of-peaks provisioning, reducing the required resources on a system level~\cite{lim2009disaggregated}.
On shared resources, \textit{interference} can cause unpredictable performance degradation of one job due to another job sharing the resources. Previous works~\cite{tzenetopoulos_interference-aware_2022,tudor_understanding_2011} on Data Center (DC) workloads have investigated such interference on shared resources, including cores, last-level caches, and memory bandwidth. In the case of a memory server, memory requests from multiple jobs will arrive at memory controllers and compete for bandwidth. High rates of memory requests can cause memory contention when there is insufficient memory bandwidth. Interference among jobs through memory contention becomes a potential runtime bottleneck, as illustrated by Figure~\ref{fig:contention}. In addition, the locality in memory accesses in a single job will be reduced when mixed with other jobs' memory requests, resulting in an unpredictable latency distribution.

\subsection{System Architecture}
two general types: distributed (split), and pool~\cite{ewais_disaggregated_2023}. We focus on Pool architecture as illustrated in Figure~\ref{fig:arch}. In particular, we target rack-scale memory pooling, where a small number of compute nodes, in tens, share memory pooling.
\begin{figure}
\centering
\includegraphics[height=3cm,width=0.9\columnwidth]{figs/arch.pdf}
\caption{A typical system architecture proposed in existing works~\cite{ewais_disaggregated_2023} and reference to LLNL Rabit with a shared memory pool providing memory resources on demand to a group of hosts/compute nodes. \todo{extend it to a tree of racks}}
\label{fig:arch}
\end{figure}


\subsection{Open Challenges}
While such systems bear similarity with heterogeneous memory systems, one main distinction is the interference from co-running  jobs. 
\textbf{Data Placement} the system architecture is essentially a multi-tier memory system composed faster tiers of local memory and slower tiers of remote memory. It poses different from existing NUMA solutions (autoNUMA in Linux is not feasible as the total memory footprint cannot fit in local tier). \todo{Common Optimizations} --> instead, this work focuses on the intrinsic algorithmic properties that stay true for scaled input problems, instead of a single application on a specific architecture to provide general optimizations. 

\textbf{Data Movement} the Unique Challenge is a composable architecture instead of a fixed one, where the interconnect bandwidth may be a variable. Two levels of granularity are commonly used -- page level and cache line. They are not mutual exclusive. Several existing works propose a hybrid of the two. \todo{Common Optimizations}--> instead, this work provides a performance model that trades off the page migration (and resulted local memory access) and remote cache line access.

\textbf{Interference and Variation} While such systems bear similarity with heterogeneous memory systems, one main distinction is the interference from co-runing  jobs. Due to multiple hosts sharing a memory pool, the system state of interference and contention could cause performance variation. \todo{Common Optimizations} --> instead, this work provides a systematic method for quantifying sensitivity to interference, and further attribute to major data objects, and identify algorithmic properties reusable on general architectures.



==> backup/design.tex <==
\section{Design and Methodology}
Our proposed framework in Figure~\ref{fig:arch} consists of four main components, namely monitoring, negotiation, migration, and control modules. For a given application, we identify selected kernels that can benefit from offloading in offline profiling. At runtime, these modules are enabled only for the selected kernels to reduce overhead. 

The overall workflow is based on the iterative nature of typical HPC applications. Many HPC applications perform simulations in iterations or time steps, each executing a set of kernels. For example, at time step $t=0$, the monitoring module collects measurements for computing the minimum resources by Algorithm~\ref{alg}. In at time $t=1$, before the start of a kernel $K$, the request tuple is sent to the memory server. If the server accepts it, the launch of $K$ will begin on near-memory cores.






==> backup/impl.tex <==
\section{Implementation}
The monitoring, control, and migrations modules were implemented as a library. The library exports two functions, \verb|nmo_start()| and \verb|nmo_stop()|, to identify the beginning and end of a target kernel. The number of available cores is set using an environment variable. The migration module calls \verb|omp_set_num_threads()| to match the number of OpenMP threads to the number of available NDP/host cores, and \verb|hwloc_set_proc_cpubind()| to set the execution mask to the emulated host or the memory server socket.

\subsection{Monitoring}
The monitoring module leverages low-level hardware performance counters. Our current implementation is based on Intel's SKX architecture, although similar capabilities are available for AMD and ARM architectures. On the host side, we use offcore events that track last-level cache miss with different submasks to local and remote DRAM
%\verb|OFFCORE_RESPONSE:L3_MISS_LOCAL| and \verb|OFFCORE_RESPONSE:L3_MISS_MISS_REMOTE_HOP1_DRAM| 
to monitor the amount of bytes accessed by a kernel. These events include all memory traffic including cache misses and account for accesses due to hardware prefetching, which can make up a majority of accesses for some numerical kernels. Our current implementation only uses aggregated counters for each kernel. In the future, we will explore fine-grained sampling within a kernel to understand the trade-off in overhead and accuracy. %Unlike oncore events such as \verb|MEM_LOCAL_L3_MISS_RETIRED|, these "offcore" events 
%On the server side, the framework monitors bandwidth usage on each memory channels. 

\subsection{Emulation Platform}



==> backup/npd.tex <==
\subsection{Opportunistic Near-memory Kernel Offloading }\label{sec:nmo}
Potential kernels are identified based on two criteria. First, only parallel regions that can leverage multiple cores will be considered because single-thread part in an HPC application should have low impact on overall execution time.


%For generality, assume an execution of a given application consists of $N$ kernels, $<k_0, k_1, ..., k_n>$. Also assume that the default memory allocation is used so that data partitioning in the local memory and memory pool remain unchanged. 

%Let $MemCap_{host}$ denote the memory capacity of the compute nodes (Host). $MemCap_{host}$ is often a constant in typical HPC systems. When the memory footprint of an application is larger than $MemCap_{host}$, the extra memory resources will be provisioned from the memory pool (memory server). We can quantify the \textit{memory composition} of an execution by the ratio between $(MemUtil_{peak} - MemCap_{host})$ and $MemUtil_{peak}$, where $MemUtil_{peak}$ is the peak memory footprint. 

 The problem is to identify which kernels would be beneficial to offloading to near-memory cores in the memory server.

In this work, only offloading is considered, i.e., a kernel either runs on host cores or near-memory cores. Co-scheduling on both host and near-memory cores is not considered to avoid potential load imbalance and the high cost of cache coherence between host and memory server~\cite{boroumand_lazypim_2016}.

The number of host cores remains constant to an application during the execution as a typical HPC job is allocated at the node boundary. However, the number of near-memory cores $N_{nmc}$ available to an application is only known at runtime, as it depends on other applications sharing the same memory server. Therefore, the offloading decision problem can be formulated as: given a kernel $K$, determine the minimum offloading cores $N_{nmc}$ to reduce the run time of $K$ compared to using the host cores, where $0<N_{nmc}\le N_{max}$.

%We re-formulate the problem into a search problem to find the minimum $N_{nmc}$ such that $T_{nmc} < T_{host}$. We first prune out compute-heavy kernels with an operational intensity above a threshold $I_{max}$, illustrated by the shaded region in the roofline model in Figure~\ref{fig:roofline}, as they cannot benefit from offloading due to the reduced computational power of the near-memory cores. After this pruning of search space, we reduce Eq.\ref{eq:1} to only consist of the memory term assuming only high $\alpha$ kernels remain.
% \begin{equation}
% \label{eq:2}
%     T = \max\Big(\frac{M_{host}}{B_{host}}, \frac{M_{pool}}{B_{pool}}\Big)
% \end{equation}

%The second pruning in the search space is to filter out kernels with $\frac{M_{host}}{B^{host}_{local}} > \frac{M_{pool}}{B^{host}_{pool}}$. Such kernels are dominated by memory access to the local memory on the compute node and offloading will have an adverse effect. The remaining kernels would have a much reduced form of Eq.~\ref{eq:1}, $T_{host} \approx \frac{M_{pool}}{B^{host}_{pool}}$. 

%By assuming the caches perform similarly on the host and the near-memory cores, we can now estimate $T_{nmc}$ based on measurements of $M_{host}$ and $M_{pool}$ on the host side---and vice versa---using Eq.~\ref{eq:2}. In future work we want to extend the model to consider also asymmetric caches.
%We leverage the following relation: $B^{p=nmc}_{remote} = B^{p=host}_{local}$,  $BW^{p=nmc}_{remote} = BW^{p=host}_{remote}$, $B^{p=nmc}_{local} = B^{p=host}_{remote}$.

%The bandwidth parameters $B_{host}$ and $B_{pool}$ can be determined by a combination of offline measurements and online monitoring. The offline measurements are carried out using microbenchmarks to quantify the peak bandwidth without interference. At runtime, the attainable bandwidth could be estimated by combining the peak bandwidth with online monitoring of the memory server and remote link. We denote bandwidth when executing on the host as $B^{host}$ and the bandwidth when executing on $N$ near-memory cores as $B^{N\times nmc}$.

\begin{comment}
    
We present Algorithm~\ref{alg} to determine the minimum required number of available offloading cores using host-local information. A resource request will be sent to the memory server, which coordinates system-wide and determines which requests to grant.

\begin{algorithm}
\caption{Find minimal number of near-memory cores}\label{alg}
\begin{algorithmic}
\Procedure{RequiredNMC}{$M_{host}, M_{pool}$}
\If{$\frac{M_{host}}{B^{host}_{local}} > \frac{M_{pool}}{B^{host}_{remote}}$}
    \State \textbf{return} $-1$
\EndIf
\State $T_{host} \gets \frac{M_{pool}}{B^{host}_{remote}}$
\For{$N \gets 1, N_{max}$}
    \State $T_{nmc} \gets \max\Big(\frac{M_{pool}}{B^{N\times nmc}_{local}}, \frac{M_{host}}{B^{N \times nmc}_{remote}}\Big)$
        \If{$T_{nmc} < T_{host}$}
        \State \textbf{return} $N$
    \EndIf
\EndFor
\State \textbf{return} $-1$
\EndProcedure
\end{algorithmic}
\end{algorithm}
\end{comment}

The compute intensity of a kernel is another factor for considering offloading. In general, near-memory cores are simpler and less powerful than host cores. Thus, they may have a lower frequency, reduced cache hierarchy, and a lower overall power budget to operate close to memory devices. We leverage the widely adopted operational intensity metric~\cite{roofline} to aggressively filter out kernels that cannot benefit from execution on near-memory cores. 

Finally, the availability of near-memory cores attached to the memory pool is only known at runtime. As the main purpose of memory pooling is to improve utilization, fixed reservation of near-memory cores to a whole job could decrease flexibility and utilization. Thus, we believe that near-memory cores should be provided on demand just like memory resources. These dynamics require negotiation mechanisms between the host and memory server, and that the availability of cores is factored into the selection of offloaded kernels.

\todo{here we need an example showing that can either (1) application benefit from offloading, (2) overall system contention is mitigated before and after offloading}

We measure the potential cost or benefit of offloading kernels in each of the workloads by relating the host execution time to the execution time with offloading for the overall application. The results are shown in Fig.~\ref{fig:offload}.

\begin{figure}
    \centering
    \includegraphics[width=\columnwidth]{figs/all_offload_px.pdf}
    \caption{Relative execution time of the applications when offloading the kernel(s) to near-memory-pool cores. The baseline is host-only execution. For NekRS, the time for the three kernels is also shown separately.}
    \label{fig:offload}
\end{figure}


%To further demonstrate the benefit of near-memory offloading for our benchmark case, we measure the memory bandwidth utilization and memory stall time for each of the configurations. The bandwidth utilization is computed from the L3 miss counters, while the memory stall time is computed as the product of the kernel execution time with the memory stall cycles ratio. Figure~\ref{fig:bw_count} shows that the bandwidth utilization increases by up to 2$\times$ as the kernel is offloaded, since it is no longer limited by the remote link. Figure~\ref{fig:stall_count} shows that the time spent waiting for the memory is reduced by 2--3$\times$ when the kernel is offloaded.



\begin{figure*}
    \centering
    \begin{subfigure}[b]{0.32\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figs/all_gl_p25_nmc12.pdf}
        \caption{25\%}
    \end{subfigure}
    \begin{subfigure}[b]{0.32\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figs/all_gl_p50_nmc12.pdf}
        \caption{50\%}
    \end{subfigure}
    \begin{subfigure}[b]{0.32\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figs/all_gl_p75_nmc12.pdf}
        \caption{75\%}
    \end{subfigure}
    \caption{Interference caused by offloaded workloads, with a varying portion of application memory footprint backed by a memory pool.}
    \label{fig:my_label}
\end{figure*}
